Petri Games: Synthesis of Distributed Systems with Causal Memory

We present a new multiplayer game model for the interaction and the flow of information in a distributed system. The players are tokens on a Petri net. As long as the players move in independent parts of the net, they do not know of each other; when they synchronize at a joint transition, each player gets informed of the causal history of the other player. We show that for Petri games with a single environment player and an arbitrary bounded number of system players, deciding the existence of a safety strategy for the system players is EXPTIME-complete.

==> eptcsdata.tex <==
\providecommand{\firstpage}{217}
\providecommand{\publicationstatus}{Adriano Peron and Carla Piazza (Eds.):\\
Proceedings of the Fifth International Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF 2014)\\
EPTCS 161, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.161.19}{10.4204/EPTCS.161.19}}

